Uncovering Vulnerable Industrial Control Systems from the Internet Core

Industrial control systems (ICS) are managed remotely with the help of dedicated protocols that were originally designed to work in walled gardens. Many of these protocols have been adapted to Internet transport and support wide-area communication. ICS now exchange insecure traffic on an inter-domain level, putting at risk not only common critical infrastructure but also the Internet ecosystem (e.g., DRDoS~attacks). In this paper, we uncover unprotected inter-domain ICS traffic at two central Internet vantage points, an IXP and an ISP. This traffic analysis is correlated with data from honeypots and Internet-wide scans to separate industrial from non-industrial ICS traffic. We provide an in-depth view on Internet-wide ICS communication. Our results can be used i) to create precise filters for potentially harmful non-industrial ICS traffic, and ii) to detect ICS sending unprotected inter-domain ICS traffic, being vulnerable to eavesdropping and traffic manipulation attacks.

==> text/authors-paperid.tex <==
\author{
  
  \IEEEauthorblockN{Paper \#~380}
}



==> text/discussion.tex <==
\section{Discussion}
\label{sec:Discussion}

There is a lack of fingerprinting tools for ICS protocols.
Given the limited deployment of ICS protocols, this comes by no surprise. We introduced and explored an advanced but lean approach to detect ICS protocols.
Our methodology is based on common Wireshark dissectors and several sanitizing steps to reduce the number of false positives. Given that we have identified ICS scanners as well as industrial ICS deployments in our traffic traces, we have trust in our true positives.

It is not surprising that inter-domain ICS traffic exist.
Internet-wide ICS scanners operate since several years. However, the amount of unprotected ICS traffic observable at central Internet vantage points is alarming.
Despite our data sanitizing steps, we found over 330k ICS packets and one anomalous traffic peak at each vantage point.

We present different characteristics for industrial and non-industrial ICS traffic. 
At the ISP, we were able to classify 98\% of the traffic as non-industrial.
At the IXP, the filtering of non-industrial traffic worked only for a subset of protocols (e.g.,BACnet).
For other protocols, we have observed a lot of industrial traffic.
Since it is a regional IXP, cooperating companies from the same country might exchange ICS traffic.
In contrast to this, our ISP data represents a transnational link between USA and Japan, representing the bridge between multiple larger, geographical distributed transit networks.
Such traffic originates at IXP-cones and is not domestic, \ie source and destination are not located in the same country.
In the future, these features can help to detect malicious activities.


==> text/relatedwork.tex <==
\section{Related Work}
\label{sec:relatedWork}

Mirian \emph{et al.}~\cite{7906943} extended an Internet-wide scanner (Zmap) by five ICS 
protocols and scanned the whole IPv4 space looking for ICS devices. They have found 60k 
exposed ICS hosts, including electrical substations or heating and ventilation systems.
They also deployed Conpot honeypot~\cite{ConpotHP} instances and evaluated 1 month 
of data from a network telescope in order to understand the behaviour of scanners.
The authors show that ICS scanning differs from broad Internet-wide scanning behaviour. 
ICS scans originate only from a handful of known actors including academic 
institutions and security firms. By providing a view into both the current 
vulnerability landscape and adversarial behaviour, the authors raise the issue of
ICS security and try to improve future protocol development.

The major differences compared to our methodology are the following.
First, by utilising passive measurements we are able detect ICS flows without creating additional ICS traffic, which reduces measurement noise. 
Second, we follow a different measurement objective.
Mirian \emph{et al.} tried to identify attackers (by using honeypots) and potential ICS devices (by scanning).
In contrast to this, our measurements try to characterize \emph{unprotected inter-domain traffic} initiated by ICS devices.
For example, we show that central internet vantage points such as IXPs have a higher coverage compared to honeypots placed in edge-networks.
In our case, we observe 37k transport layer requests on ICS ports at two 
honeypot sensors, but identify 330k sanitized ICS flows at the IXP and ISP.
We confirm that ICS scans are run by a handful of organizations and that
ICS devices have become a popular scanning target since the beginning of 2014.
Utilizing the central vantage points, we are also able to describe how topological
properties of non-industrial traffic look like, allowing an early risk assessment.
Additionally, we see if hosts answer selectively to ICS traffic and if they exchange 
unprotected ICS traffic with other ICS hosts, potentially being susceptible to 
eavesdropping.

BACnet has been studied before at central Internet vantage points. 
Gasser \emph{et al.} \cite{gasser2017amplification} evaluate the vulnerability of
BACnet to DDoS amplification attacks by active scanning and passive traffic measurements
at an ISP and IXP. They find 16k BACnet devices and more than 14k of these devices can 
be misused as amplifiers, with amplification factors up to 120.
The authors perform a port-based detection of ICS traffic at the IXP and observe
a large number of small sized scanning packets, typically around 45 to 70 bytes.
The authors analyse BACnet traffic from the same ISP as we have, however, they choose a special 
full-trace spanning over 48 hours, instead of providing a long-term study over six months.
They pre-filter the data set by ports, then
fingerprint the payload with a self-written script by checking the first bytes of
the UDP payload. Surprisingly, they only find four different payloads in over 335k
BACnet request packets, which hints at scanning activities instead of industrial 
traffic.

Based on our results, we confirm heavy BACnet scanning at the IXP and ISP.
In contrast to previous work, our analysis also checks the packet payload at the IXP, which makes the results more accurate.
Furthermore, we explore the potentials of common open source tools and introduce a lean methodology to achieve both sanitizing of the captured data and distinction between industrial and non-industrial ICS traffic.
Most importantly, in this paper we present the first in-depth, longitudinal traffic analysis of multiple ICS protocols.

